Matched-filter study and energy budget suggest no detectable gravitational-wave 'extended emission' from GW170817

Van Putten & Della Valle (2018) have reported a possible detection of gravitational-wave 'extended emission' from a neutron star remnant of GW170817. Starting from the time-frequency evolution and total emitted energy of their reported candidate, we show that such an emission is not compatible with the current understanding of neutron stars. We explore the additional required physical assumptions to make a full waveform model, for example, taking the optimistic emission from a spining-down neutron star with fixed quadrupolar deformation, and study whether even an ideal single-template matched-filter analysis could detect an ideal, fully phase-coherent signal. We find that even in the most optimistic case an increase in energy and extreme parameters would be required for a confident detection with LIGO sensitivity as of 2018-08-17. The argument also holds for other waveform models following a similar time-frequency track and overall energy budget. Single-template matched filtering on the LIGO data around GW170817, and on data with added simulated signals, verifies the expected sensitivity scaling and the overall statistical expectation.

==> makefile <==
DOCS := resvp.pdf

EXTRA_TEX = 

TABLES = 

MANUAL_FIGURES = xMC2-SNR-Pdet-Ieps.pdf \
	PFD-PFA-RHOopt.pdf \
	pycbc_vP_SNR_timeseries.pdf \
	pycbc_vP_SNR_timeseries_hists.pdf \
	pyCBC_SNR_vs_Egw_Msun_vPinj_H1_L1.pdf \
	alt_models_fgw_h0_Egw.pdf

AUTO_FIGURES   =

BIBLIO = ../resvp.bib

BYPROD = *.aux *.log *.out *.dvi *.blg *.bbl *~ __tmp *Notes.bib

default: gitID $(DOCS)

.PHONY : gitID
gitID:
	
	cd .. && chmod +x git-tag.sh && ./git-tag.sh && cd paper

resvp.pdf: resvp.tex resvp.bbl $(EXTRA_TEX) $(BIBLIO) $(AUTO_FIGURES) $(MANUAL_FIGURES) $(TABLES) ../gitID.txt
	pdflatex $(@:.pdf=) && pdflatex $(@:.pdf=)

resvp.bbl: $(BIBLIO)
	pdflatex $(@:.bbl=) && bibtex $(@:.bbl=)

clean:
	rm -f $(DOCS) $(BYPROD) gitID.txt

